Habitat-Matterport 3D Semantics Dataset

We present the Habitat-Matterport 3D Semantics (HM3DSEM) dataset. HM3DSEM is the largest dataset of 3D real-world spaces with densely annotated semantics that is currently available to the academic community. It consists of 142,646 object instance annotations across 216 3D spaces and 3,100 rooms within those spaces. The scale, quality, and diversity of object annotations far exceed those of prior datasets. A key difference setting apart HM3DSEM from other datasets is the use of texture information to annotate pixel-accurate object boundaries. We demonstrate the effectiveness of HM3DSEM dataset for the Object Goal Navigation task using different methods. Policies trained using HM3DSEM perform outperform those trained on prior datasets. Introduction of HM3DSEM in the Habitat ObjectNav Challenge lead to an increase in participation from 400 submissions in 2021 to 1022 submissions in 2022.

==> sections/checklist.tex <==
\section{NeurIPS 2021 Paper Checklist}

For all authors...

(a) Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? Yes.

(b) Have you read the ethics review guidelines and ensured that your paper conforms to them? Yes

(c) Did you discuss any potential negative societal impacts of your work? Yes. We discuss potential biases in the dataset in Section S1 of \code{supplementary.pdf}.

(d) Did you describe the limitations of your work? Yes. We discuss limitations in the dataset and annotations in Section S1 in \code{supplementary.pdf}.

If you ran experiments...

(a) Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? Yes. The dataset is publicly available at {\small \url{https://github.com/facebookresearch/habitat-sim/blob/master/DATASETS.md}}. Please see \code{submission\_code} directory in \code{supplementary.zip} for the code and instructions.

(b) Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? Yes. Please see Section S2 in \code{suppplementary.pdf}.

(c) Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? Yes. We report the mean and standard-deviation by evaluating the same model over 3 random seeds (see Table 2 in main paper). We do not train our model over multiple random seeds due to high computational requirements.

(d) Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? Yes. Please see Section S3 in \code{supplementary.pdf}.


If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...

(a) If your work uses existing assets, did you cite the creators? Yes. Our dataset uses new, unique assets not previously used in any dataset. We have cited all baselines which use external code or datasets.

(b) Did you mention the license of the assets? Yes. We are including specific license, copyright information and terms of use in the packaging for our new Habitat-Matterport 3D. Please see Section S4 in \code{supplementary.pdf}.

(c) Did you include any new assets either in the supplemental material or as a URL? Yes. This paper introduces our new Habitat-Matterport 3D dataset. Please see Section S4 in \code{supplementary.pdf}.

(d) Did you discuss whether and how consent was obtained from people whose data you're using/curating? Yes. We obtained consent from users for curating the HM3D dataset. See Section S5 in \code{supplementary.pdf}. 

(e) Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? Yes. Matterport used a commercially reasonable effort to try and obscure such information. See Section S5 in \code{supplementary.pdf} for a detailed overview.

% All Habitat Matterport 3D models are constructed from a series of panoramas. We manually checked all panoramas from which the data was constructed for PII information.  For any we did find, we either discarded the scene from the dataset or blurred the offending region of the panorama. If the panorama was altered, we reran our reconstrution pipeline on the mesh.
% Please see Section S5 in \code{supplementary.pdf}.


% (a) Did you include the full text of instructions given to participants and screenshots, if applicable?

% Including this information in the supplemental material is fine, but if the main contribution of your paper involves human subjects, then we strongly encourage you to include as much detail as possible in the main paper.

% (b) Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?

% Examples of risks include a crowdsourcing experiment which might show offensive content or collect personal identifying information (PII). Ideally, the participants should be warned.

% Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.  For initial submissions, do not include any information that would break anonymity, such as the institution conducting the review.

% (c) Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?

% First, provide the amount paid for each task (including any bonuses), and discuss how you determined the amount of time a task would take.

% Also include discussion on how the wage was determined and how you determined that this was a fair wage.

==> sections/other_licences.tex <==
\section{Licenses for referenced datasets}
Gibson: {\small\url{http://svl.stanford.edu/gibson2/assets/GDS_agreement.pdf}}\\
Matterport3D: {\small\url{http://kaldir.vc.in.tum.de/matterport/MP_TOS.pdf}} \\
ScanNet: \small{\url{http://kaldir.vc.in.tum.de/scannet/ScanNet_TOS.pdf}} \\
Replica: \small{\url{https://github.com/facebookresearch/Replica-Dataset/blob/master/LICENSE}}
